Tropical Logistic Regression Model on Space of Phylogenetic Trees

Classification of gene trees is an important task both in the analysis of multi-locus phylogenetic data, and assessment of the convergence of Markov Chain Monte Carlo (MCMC) analyses used in Bayesian phylogenetic tree reconstruction. The logistic regression model is one of the most popular classification models in statistical learning, thanks to its computational speed and interpretability. However, it is not appropriate to directly apply the standard logistic regression model to a set of phylogenetic trees, as the space of phylogenetic trees is non-Euclidean and thus contradicts the standard assumptions on covariates. It is well-known in tropical geometry and phylogenetics that the space of phylogenetic trees is a tropical linear space in terms of the max-plus algebra. Therefore, in this paper, we propose an analogue approach of the logistic regression model in the setting of tropical geometry. Our proposed method outperforms classical logistic regression in terms of Area under the ROC Curve (AUC) in numerical examples, including with data generated by the multi-species coalescent model. Theoretical properties such as statistical consistency have been proved and generalization error rates have been derived. Finally, our classification algorithm is proposed as an MCMC convergence criterion for Mr Bayes. Unlike the convergence metric used by MrBayes which is only dependent on tree topologies, our method is sensitive to branch lengths and therefore provides a more robust metric for convergence. In a test case, it is illustrated that the tropical logistic regression can differentiate between two independently run MCMC chains, even when the standard metric cannot.

==> fw_points.tex <==
\begin{proof}[{\bf Proof of Proposition 
\ref{prop:consistency_of_Fermat_Weber_points}}]
Consider the random variable 
$d_{\rm tr}(X,\alpha)$. From the triangular inequality 
\begin{equation*}
    d_{\rm tr}(X,\alpha) \leq 
    d_{\rm tr}(X,\omega^*) + 
    d_{\rm tr}(\alpha,\omega^*),
\end{equation*}
it is deduced that $d_{\rm tr}(X,\alpha)$ is integrable, bounded
above by an integrable random variable. 
\par 
Now consider the function 
% $F: \mathbb{R}^e/ \mathbb{R}{\bf 1}$ 
$F: \trtor \to \R$,
\[
    F(x) = d_{\rm tr}(x,\omega) + 
    d_{\rm tr}(2\omega^* - x,\omega) - 
    2d_{\rm tr}(x,\omega^*).
\]
Noting that 
$d_{\rm tr}(2\omega^* - x,\omega) 
= d_{\rm tr}(x,2\omega^* - \omega)$,
it follows that $F(X)$ is integrable as the sum of integrable 
random variables.
\par 
From triangular inequality 
and the fact that $d_{\rm tr}(2\omega^* - x,x) = 2d_{\rm tr}(x,\omega^*)$
it follows that 
$F(x) \geq 0$ for all $x \in \trtor$.
Furthermore, $F(\omega^*)>0$ and since $F$ is continuous, there 
exists a neighbourhood $U$ that contains $\omega^*$ such that 
$F(x) > 0$ for all $x \in U$. Moreover, 
the function has positive density in a neighbourhood $V$ 
that contains the centre $\omega^*$. Therefore, there exists 
a neighbourhood $W = U \cap V$ such that $F(x) > 0$ for all 
$x \in W$ and $\mathbb{P}(X \in W) > 0$. Hence, since 
$F(X) \geq 0$, 
\begin{equation*}
    \mathbb{E}(F(X)) 
    \geq 
    \mathbb{E}(F(X)| X \in W) \mathbb{P}(X \in W ) > 0. 
\end{equation*}
In other words, 
\begin{equation}
    \label{ineq:EF>0}
    \mathbb{E}\left(d_{\rm tr}(X,\omega)\right) + 
    \mathbb{E}\left(d_{\rm tr}(2\omega^*-X,\omega)\right) >  
    2 \mathbb{E}(d_{\rm tr}(x,\omega^*))
\end{equation}
Moreover, consider the isometry $y = 2\omega^*-x$ 
and note that for symmetric probability 
density functions around $\omega^*$, 
$f(\omega^*-\delta) = f(\omega^* + \delta)$ and so for 
$\delta = \omega^* - x$, we have $f(y)=f(x)$. 
Applying this transformation to the following integral yields
\begin{align}
    \mathbb{E}(d_{\rm tr}(2\omega^* - X,\omega)) &= 
    \int_{\trtor} d_{\rm tr}(2\omega^* - x,\omega) f(x) \, dx  
    \label{eq:2omega-x} \\ & =
    \int_{\trtor} d_{\rm tr}(y,\omega) f(y) \, dy 
    = \mathbb{E}(d_{\rm tr}(X,\omega)). \nonumber
\end{align}
Combining equation \eqref{eq:2omega-x} with inequality 
\eqref{ineq:EF>0} shows that the function 
$Q(\omega) = \mathbb{E}(d_{\rm tr}(X,\omega))$ 
has a global minimum at $\omega^*$.
\par 
From Theorem \ref{thm:uniform_law_of_large_numbers} (uniform
law of large numbers), set 
$f(x,\omega) = d_{\rm tr}(x,\omega)$ and observe that 
$f(x,\omega)$ is always continuous w.r.t. $\omega$. 
Setting 
$r(x) = \sup_{\omega \in \Omega} d_{\rm tr}(x,\omega)$, which 
is finite since $\Omega$ is compact, observe that
\[
    r(x) := \sup_{\omega \in \Omega} d_{\rm tr}(x,\omega)
    \leq d_{\rm tr}(x,\omega^*) + 
    \sup_{\omega \in \Omega} d_{\rm tr}(\omega,\omega^*).
\]
Since $\Omega$ is compact, the second term is finite and hence 
$r(X)$ is integrable, since $d_{\rm tr}(X,\omega^*)$ is
integrable. All conditions of the theorem are satisfied so 
$Q(\omega) = \mathbb{E}(d_{\rm tr}(x,\omega))$ is continuous 
with respect to $\omega$ and 
\begin{equation*}
        \sup_{\omega \in \Omega} 
        |Q_n(\omega) - Q(\omega)| 
        \overset{p}{\to}
        0 \text{ as }
        n \to \infty, 
\end{equation*}
where $Q_n(\omega) = n^{-1} \sum_{i=1}^n d_{\rm tr}(X_i,\omega)$. 
Since $Q(\omega)$ has a unique minimum at $\omega^*$, all 
conditions of Theorem 
\ref{thm:convergence_of_theta_n} are satisfied and so 
$\Tilde{\omega}_n \to \omega^*$ as $n \to \infty$.
\end{proof}

\begin{proof}[{\bf Proof of Proposition \ref{prop:vanishing_gradient}}]
\begin{enumerate}[i.]
    \item If $\omega - X_i$ has a unique maximum 
    $M_i = \argmax_j\{\omega_j - (X_i)_j\}$ and 
    unique minimum 
    $m_i = \argmin_j\{\omega_j - (X_i)_j\}$, then the 
    gradient is
    \begin{equation}
        \label{eq:gradient_f}
        (\nabla f(x))_j = |\{i: M_i=j\}| - |\{i: m_i=j\}|.
    \end{equation}
    For the converse, assume that the gradient is 
    well-defined. From equations 
    \eqref{eq:dtr_pos}--\eqref{eq:dtr_neg} and following the 
    first few sentences of Lemma 
    \ref{lemma:uniqueness_of_optimum}
    \[d_{\rm tr}(x+\epsilon E_j,y) +
    d_{\rm tr}(x-\epsilon E_j,y) - 
    2d_{\rm tr}(x,y) = \epsilon s_j(x-y), 
    \]
    where $s_j$ is defined in equation \eqref{eq:s_i} of 
    Lemma \ref{lemma:uniqueness_of_optimum}.
    Consequently,
    \[
    f(x+\epsilon E_j) + f(x- \epsilon E_j) -
    2f(x) = \epsilon \sum_{i=1}^n s_j(X_i - \omega_i)
    \]
    Since $f$ has a well-defined gradient, 
    $\sum_{i=1}^n s_j(X_i - \omega) = 0$
    i.e. $s_j(X_i - \omega) = 0$ for all 
    $(i,j) \in [n] \times [e]$. This can only happen iff 
    $X_i - \omega$ has unique maximum and minimum component 
    for all $i \in [n]$.
    \item Using equation \eqref{eq:gradient_f}, the gradient 
    of $f$ vanishes at $x=\omega$ if and only if
    \begin{equation}
        \label{eq:vanishing_gradient}
        |\{i: M_i=j\}| = |\{i: m_i=j\}|.
    \end{equation}
    Moreover,
    \begin{align*}
        f(\omega+v) &= \sum_{i=1}^n 
        \max_k \left\{ \omega_k - (X_i)_k + v_k \right\} - 
        \min_k \left\{ \omega_k - (X_i)_k + v_k \right\}\\ 
        & \geq 
        \sum_{i=1}^n 
        \omega_{M_i} - (X_i)_{M_i} + v_{M_i} - 
        \omega_{m_i} + (X_i)_{m_i} - v_{m_i} \\ 
        & = 
        f(\omega) + \sum_{i=1}^n v_{M_i} - v_{m_i}
    \end{align*}
    Finally, note that because of equation 
    \eqref{eq:vanishing_gradient}, 
    \begin{align*}
        \sum_{i=1}^n v_{M_i} &= \sum_{j=1}^e 
        v_j |\{i \in [n]:M_i=j\}| \\ &
        \overset{\eqref{eq:vanishing_gradient}}{=} 
        \sum_{j=1}^e 
        v_j |\{i \in [n]:m_i=j\}| = 
        \sum_{i=1}^n v_{m_i},
    \end{align*}
    and so $f(\omega+v) \geq f(\omega)$ for all 
    $v \in \trtor$. 
\end{enumerate}

\end{proof}



==> gen_error.tex <==
\begin{proof}[{\bf Proof of Proposition 
\ref{prop:gen_error_one_species}}]
First, define $\Delta_0 = \{ C(X) \neq 1  | Y = 0 \} $. 
By definition of $C(X)$, 
\begin{align*}
    \Delta_0 &= \left\{ \left. (\sigma_0^{-1} - \sigma_1^{-1}) d_{\rm tr}(X,\Hat{\omega})
    - (e-1) \log{\left( \frac{\sigma_1}{\sigma_0}  \right)} \geq 0
    \right| Y=0 
    \right\}\\
    & = 
    \left\{ \left.
    d_{\rm tr}(X,\Hat{\omega}) \geq \alpha \sigma_0 \sigma_1 
    \right| Y=0 
    \right\}.
\end{align*}
Triangular inequality dictates that 
\begin{equation*}
    d_{\rm tr}(X,\omega^*) - d_{\rm tr}(\omega^*,\Hat{\omega}) 
    \leq 
    d_{\rm tr}(X,\Hat{\omega}) 
    \leq 
    d_{\rm tr}(X,\omega^*) + d_{\rm tr}(\omega^*,\Hat{\omega}), 
\end{equation*}
and so it follows that 
\begin{align*}
    \Delta_0 & \supseteq 
    \{ d_{\rm tr}(X,\omega^*) \geq \sigma_0 \sigma_1 \left( \alpha + \epsilon  \right) | Y = 0  \} \\ 
    \Delta_0 & \subseteq
    \{ d_{\rm tr}(X,\omega^*) \geq \sigma_0 \sigma_1 \left( \alpha - \epsilon  \right) | Y = 0  \}, 
\end{align*}
and since $Z = \sigma_0^{-1} d_{\rm tr}(X,\omega^*)|Y=0\sim F$, 
\begin{equation*}
    \mathbb{P}( Z \geq \sigma_1 (\alpha + \epsilon)) \leq
    \mathbb{P}(\Delta_0) \leq
    \mathbb{P}( Z \geq \sigma_1 (\alpha - \epsilon)),
\end{equation*}
which yields the desired result.\\
Similarly, for $\Delta_1 = \{ C(X) \neq 0 | Y = 1 \} = 
\left\{ d_{\rm tr}(X,\Hat{\omega}) \leq \sigma_0 \sigma_1 \alpha \right\}$,
\begin{align*}
    \Delta_1 & \supseteq 
    \{ d_{\rm tr}(X,\omega^*) \leq \sigma_0 \sigma_1 \left( \alpha - \epsilon  \right) | Y = 1  \} \\ 
    \Delta_1 & \subseteq
    \{ d_{\rm tr}(X,\omega^*) \leq \sigma_0 \sigma_1 \left( \alpha + \epsilon  \right) | Y = 1  \}, 
\end{align*}
and since $Z = \sigma_1^{-1} d_{\rm tr}(X,\omega^*)|Y=1\sim F$, 
\begin{equation*}
    \mathbb{P}( Z \leq \sigma_0 (\alpha - \epsilon)) \leq
    \mathbb{P}(\Delta_1) \leq
    \mathbb{P}( Z \leq \sigma_0 (\alpha + \epsilon)),
\end{equation*}
which is the desired interval. \\
For the second part of the proposition, $\Hat{\omega} = \omega^*$ and so 
$\epsilon = 0$. Hence, 
\begin{align*}
    \mathbb{P}(\Delta_0) &= 1 - F(\sigma_1 \alpha ) = 1- F( x u(x) ) \\ 
    \mathbb{P}(\Delta_1) &= F(\sigma_0 \alpha ) = F( u(x) ), \text{ where } \\ 
    x = \frac{\sigma_1}{\sigma_0} & \text{ and }
    u(x) = (e-1) \frac{ \log{x} }{x - 1}   
\end{align*}
Consider the function 
\[g(x) = 1-F(xu(x)) - F(u(x))\]
Proving that $g(x) <0 $ for all $x > 1$ is equivalent to proving 
the desired result that 
$\mathbb{P}(\Delta_0) < \mathbb{P}(\Delta_1)$ for $\sigma_1 > \sigma_0$. 
First, 
\begin{equation*}
    \lim_{x \to 1} u(x) = \lim_{x \to 1} x u(x) = e-1,
\end{equation*}
and so $\lim_{x \to 1} g(x) = 1-2F(e-1)$. 
It is a well-known fact that the median of the ${\rm Gamma}$ distribution is less than
the mean. 
Hence, for $Z \sim {\rm Gamma}(e-1,1)$ with mean $e-1$,
$F(e-1) > \frac{1}{2}$ and so 
\begin{equation}
    \label{eq:limx_g}
    \lim_{x \to 1} g(x) < 0.
\end{equation}
Finally, the derivative of $g$ is 
\begin{equation*}
    g'(x) = 
    - F'(u(x)) u'(x) - F'(xu(x)) (xu'(x) + u(x)) 
\end{equation*}
The following two inequalities 
\begin{align}
    F'(u(x))  \geq F'(xu(x)), & \label{eq:F'} \\
    u'(x) + xu'(x) + u(x) & \geq 0, \label{eq:u'}
\end{align}
imply that 
\begin{equation}
    \label{eq:g'}
    g'(x) \leq 
    - F'(xu(x)) (u'(x) + xu'(x) + u(x))
    \leq 0.
\end{equation}
From \eqref{eq:limx_g} and \eqref{eq:g'} 
it follows that $g(x) < 0$ for all $x>1$.\\
For inequality \eqref{eq:F'}, remember that 
\begin{equation*}
    F'(x) = \frac{x^{e-2} \exp{(-x)} }{\Gamma(e-1)}
\end{equation*}
and so 
\begin{align*}
    F'(u(x)) - F'(xu(x)) &=  
    F'(u(x))
    \left(
        1 - x^{e-2}  \exp(-(x-1) u(x))
    \right) \\ &=
    F'(u(x))
    \left(
        1 - x^{e-2}  \exp(-(e-1) \log(x))
    \right) \\ &= 
    F'(u(x))(1-x^{-1})>0,
\end{align*}
for all $x>1$.\\ 
For inequality \eqref{eq:u'},
\begin{equation*}
     u'(x) + xu'(x) + u(x) = \frac{e-1}{(x-1)^2} \left( x-x^{-1} -2\log{x} \right),
\end{equation*}
is a non-negative function for $x>1$
iff $v$ is a non-negative function, where
\begin{align*}
    v(x) & = x - x^{-1} - 2\log{x}, \text{ with } \\
    v'(x) & = \frac{(x-1)^2}{x^2} \geq 0
    \text{ and } 
    v(1) = 0. 
\end{align*}
Clearly, $v$ is a non-negative function
for $x>1$, so 
inequality \eqref{eq:u'} is satisfied.
\end{proof}

\begin{proof}[{\bf Proof of Proposition 
\ref{prop:gen_error}}]
    For symbolic convenience, in this proof class $0$ is referred to as class $-1$ 
    and so $Y \in \{-1,1\}$.
    Applying the triangular inequality twice, 
    \begin{align*}
        D_X &
        = d_{\rm  tr}(X , \omega^*_Y)  - d_{\rm  tr}(X , \omega^*_{-Y}) 
        \\ & \geq 
        \left( 
            d_{\rm  tr}(X , \Hat{\omega}_Y) - d_{\rm  tr}(  \omega^*_Y , \Hat{\omega}_Y )  
        \right) \\& - \left(
            d_{\rm  tr}(X , \Hat{\omega}_{-Y}) + d_{\rm  tr}(  \omega^*_{-Y} , \Hat{\omega}_{-Y} )  
        \right) \\
        &= 
        d_{\rm  tr}(X , \Hat{\omega}_Y) - d_{\rm  tr}(X , \Hat{\omega}_{-Y}) - \epsilon, 
    \end{align*}
    it follows that
    \[
    \{ C(X) \neq Y \} =
    \{d_{\rm  tr}(X , \Hat{\omega}_Y)  - d_{\rm  tr}(X , \Hat{\omega}_{-Y})
        \geq 0\}  \subseteq \{D_X \geq - \epsilon\}
    \] 
    and so 
    the generalization error has the following upper bound
    \begin{equation*}
        \mathbb{P}( C(X) \neq Y ) 
        \leq 
        \mathbb{P} \left( D_X \geq -\epsilon \right).
    \end{equation*}
    Note that if 
    $d_{\rm tr}(X,\omega_Y^*) < \Delta_\epsilon$, 
    then by the use of triangular inequality 
    \begin{align*}
         D_X & =d_{\rm  tr}(X , \omega^*_Y)  - d_{\rm  tr}
         (\omega^*_{-Y},X) 
         \\ & \leq 
         d_{\rm  tr}(X , \omega^*_Y) - \left(
            d_{\rm  tr}(\omega_{-Y}^*, \omega_Y^* ) -d_{\rm  tr}
            (\omega^*_Y,X) 
         \right)
         \\ &
         < 2\Delta_{\epsilon}-d_{\rm  tr}(\omega_1^* , \omega_{-1}^*) = -\epsilon. 
    \end{align*}
    % Conditioning on the sign of $Z-\Delta_\epsilon$, 
    Consequently, 
    \begin{equation}
        \label{eq:gen_error_leq_DXZX}
        \mathbb{P}( C(X) \neq Y )  \leq 
        \mathbb{P}\left( D_X \geq -\epsilon , 
        Z_X \geq \Delta_\epsilon
        \right) 
    \end{equation}
    Since the distribution of $X$ is symmetric around 
    $\omega^*_Y$, the random variable 
    $2\omega^*_Y - X$ has the same distribution and so 
    \begin{equation}
        \label{eq:gen_error_2omega-X}
        \mathbb{P}\left( D_X \geq -\epsilon , 
        Z_X \geq \Delta_\epsilon
        \right) = \mathbb{P}\left( D_{2\omega_Y^*-X} \geq -\epsilon , 
        Z_{2\omega_Y^*-X} \geq \Delta_\epsilon
        \right). 
    \end{equation}
    It will be proved that 
    \begin{align}
        Z_{2\omega_Y^*-X} &= Z_{X}, \label{eq:Z} \\ 
        D_X + D_{2\omega_Y^*-X} &\leq 0, \label{eq:D}
    \end{align}
    and so 
    $\{D_{2\omega_Y^*-X} \geq -\epsilon , 
        Z_{2\omega_Y^*-X} \geq \Delta_\epsilon\} \subseteq 
    \{D_{X} \leq \epsilon , 
    Z_{X} \geq \Delta_\epsilon\}.
    $
    Then, using equation \eqref{eq:gen_error_2omega-X}, 
    \begin{equation*}
    \mathbb{P}\left( D_X \geq -\epsilon , 
        Z_X \geq \Delta_\epsilon
        \right)
    \leq  
    \mathbb{P}\left(D_{X} \leq \epsilon , 
    Z_{X} \geq \Delta_\epsilon\right),
    \end{equation*}
    and substituting it to inequality 
    \eqref{eq:gen_error_leq_DXZX},
    \begin{align*}
        \mathbb{P}(C(X) \neq Y)) = & 
        \frac{1}{2} ( \mathbb{P}\left( D_X \geq -\epsilon , 
        Z_X \geq \Delta_\epsilon
        \right)  \\ + & \,\,\,\,
        \mathbb{P}\left( D_X \leq \epsilon , 
        Z_X \geq \Delta_\epsilon
        \right) 
	) \\ = &  
        \mathbb{P}\left( 
            Z_X \geq \Delta_\epsilon
        \right) + h(\epsilon) 
    \end{align*}
    where $h(\epsilon) = 
    \mathbb{P}(Z_X \geq \Delta_\epsilon, |D_X| \leq \epsilon)$
    is an increasing function with respect to $\epsilon$, 
    which completes the proof.\\
    Equation \eqref{eq:Z} follows from the observation that
    \[d_{\rm tr}(2\omega_Y^*-x,\omega_Y^*) = 
    d_{\rm tr}(x,\omega_Y^*).\]
    For equation \eqref{eq:D},
    \begin{align*}
        D_{2\omega_Y^*-X} + D_X &=
        Z_{2\omega_Y^*-X} 
        - d_{\rm  tr}( 2 \omega_Y^* - X , \omega_{-Y}^* )  \\&
        + Z_X
        - d_{\rm  tr}(X,\omega_{-Y}^*) \\ &
        \overset{\eqref{eq:Z}}{=}
        2Z_{2\omega_Y^*-X}  -  
            d_{\rm  tr}( 2 \omega_Y^* - X,  \omega_{-Y}^* ) -
            d_{\rm  tr}(\omega_{-Y}^*,X)
         \\ 
        & \leq 
        2Z_{2\omega_Y^*-X}  -  
            d_{\rm  tr}( 2 \omega_Y^* - X,  X ) 
        = 0,
    \end{align*}
    where the last inequality comes from the triangular inequality.
\end{proof}

==> other.tex <==
\section{Fermat-Weber Point Visualization} \label{sec:fw_point_illustration}
As noted in Section \ref{sec:optimization}, the
gradient method is much faster than 
linear programming. Unfortunately, there is no guarantee
that it will guide us to a Fermat-Weber point. 
However, in practice, the gradient method tends to work 
well. Figure \ref{fig:fw_vis} illustrates just that.
Given, ten datapoint $X_1, \dots, X_{10} \in 
\mathbb{R}^3/\mathbb{R}{\bf 1} \cong \mathbb{R}^2$,
the Fermat-Weber set is found to be a trapezoid.  
This is in agreement with 
\cite{lin2018tropical}, which 
states that all Fermat-Weber sets are 
classical polytopes. The two-dimensional gradient 
vector, plotted as a vector field in Figure 
\ref{fig:fw_vis}, 
always points towards the Fermat-Weber set. 
Therefore, the gradient algorithm should always guide us
to a Fermat-Weber point. 
\begin{figure}[h]
    \centering
    \includegraphics[width=.9\linewidth]{fermat_weber_illustration.eps}
    \caption{Visualization of the function 
    $f(\omega)= \sum_{i=1}^{10} d_{\rm tr}(X_i,\omega)$
    for $X_i$. The black circles are
    the datapoints $X_1, \dots, X_{10}$, 
    the solid lines are contours of $f$, the vector
    field is the gradient and the small black trapezoid
    at $(0.65,0.55)$ is the Fermat-Weber set.
    }
    \label{fig:fw_vis}
\end{figure}
\section{MLE Estimator for $\sigma$}
If $Z_i \overset{\rm iid}{\sim} {\rm Gamma}(n, k)$,  
where $n$ is constant and $k$ is a statistical parameter, then 
it is well-known that
the maximum likelihood estimator is 
\begin{equation}
    \label{eq:bar_k}
    \Hat{k} = \Bar{Z}/n,
\end{equation}
where $\Bar{Z}$ is the sample average. 
In our case $Z_i = d(X_i,\omega^*)$ and $k= i \sigma^i$.
From Proposition \ref{prop:tropical_radius_dist}, 
$Z_i \sim {\rm Gamma}(n/i,i\sigma^i)$ 
and by substituting these parameters in equation \ref{eq:bar_k},
it follows that the MLE for $\sigma$ is
\[
    \Hat{\sigma}^i = \Bar{Z} / n,
\]
where $\Bar{Z}$ is the average distance of the covariates (gene trees) 
from their mean (species tree). 
This results holds for all $i \in \mathbb{N}$ and both Euclidean and 
tropical metrics. The only difference is that 
for Euclidean spaces $X \in \mathbb{R}^e$ and so $n=e$, while for 
the tropical projective torus $\trtor$, $n=e-1$.
\section{Approximate BHV Logistic Regression}
Similar to the tropical Laplace distribution, in \cite{BHV} the following 
distribution was considered
\begin{equation*}
    f_{\lambda,\omega}(x) = K_{\lambda,\omega} \exp\left(-\lambda d_{\rm BHV}(x,\omega) \right),
\end{equation*}
where $\lambda = 1/\sigma$ is a concentration/precision parameter,
$d_{\rm BHV}$ is the BHV metric and $K_{\lambda,\omega}$ is the normalization 
constant that depends on $\lambda$ and $\omega$.
We consider an adaptation of the two-species model for this metric, where 
the data from the two classes have the same concentration rate but different 
centre.
If $X|Y \sim f_{\lambda,\omega^*_Y}$, then 
\begin{equation}
    \label{eq:bhv_logistic_regression}
    h_{\omega_0,\omega_1}(x) =
    \lambda \left(
        d_{\rm BHV}(x,\omega_0^*) -  d_{\rm BHV}(x,\omega_1^*)
    \right) + 
    \log{\frac{K_{\lambda,\omega^*_0 }}{K_{\lambda,\omega^*_1}}}.
\end{equation}
Unlike in the tropical projective torus or the euclidean space, in the BHV space
$K_{\lambda,\omega^*_0 } \neq K_{\lambda,\omega^*_1}$, because the space
is not translation-invariant.
However, if we assume that the two centres are far away from trees with 
bordering topologies, it may be assumed that the trees are mostly distributed 
in the Euclidean space and as a result 
$K_{\lambda,\omega^*_0 } \approx K_{\lambda,\omega^*_1}$. 
Under this assumption, equation \eqref{eq:bhv_logistic_regression}
becomes
\begin{equation*}
    h_{\omega_0,\omega_1}(x) \approx
    \lambda \left(
        d_{\rm BHV}(x,\omega_0^*) -  d_{\rm BHV}(x,\omega_1^*)
    \right). 
\end{equation*}
Therefore, the classification/decision boundary for the BHV is the 
BHV bisector $d_{\rm BHV}(x,\omega_0^*) =  d_{\rm BHV}(x,\omega_1^*)$
and the most sensible classifier is 
\begin{equation*}
    C(x) = \mathbb{I}\left(d_{\rm BHV}(x,\omega_0^*) >  
    d_{\rm BHV}(x,\omega_1^*)\right),
\end{equation*}
where $ \mathbb{I}$ is the indicator function.

\section{Graphs for Simulated Data under the Multi-Species Coalescent Model for different $R$}
\label{sec:coalescent_graphs}
\begin{figure}[h]
    \centering
    \includegraphics[width=.49\linewidth]
    {rfdist_hist.eps}
    \includegraphics[width=.49\linewidth]
    {trop_dists_hist_Rs.eps}
    \caption{(LEFT) Robinson-Foulds distances 
    and (RIGHT) tropical distances of inferred species
    trees $\Hat{\omega}$ from the 
    actual species trees $\omega^*$ for 
    $R=0.1,1,10$.}
    \label{fig:dist_hists}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{rocs.eps}
    \caption{ROC curves for the tropical logistic regression with different values of $R$.  Higher the value of $R$ is the closer an estimated ROC curve for the tropical logistic regression model gets to the point $(0, 1)$. }
    \label{fig:rocs}
\end{figure}


==> pseudocode.tex <==
\section{Tropical Logistic Regression Algorithm} \label{sec:alg}

\begin{algorithm}
\caption{One-species tropical logistic regression}\label{alg:one}
\begin{algorithmic}
\State {\bf Input: } distance matrix $D \in \mathbb{R}_+^{N \times e}$, labels $Y \in \{0,1\}^{N}$ 
\State $\Tilde{\omega} = {\rm FW\_point}(D)$
\State $\Hat{\sigma}_0, \Hat{\sigma}_1 = \argmax_{\sigma_0,\sigma_1 > 0} l(\Tilde{\omega},\sigma_0,\sigma_1)| D,Y)$ with root solving.
\State {\bf Output: } $(\Tilde{\omega},\Hat{\sigma}_0,\Hat{\sigma}_0 )$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Two-species tropical logistic regression}\label{alg:two}
\begin{algorithmic}
\State {\bf Input: } distance matrix $D \in \mathbb{R}_+^{N \times e}$, labels $Y \in \{0,1\}^{N}$ 
\State $\Tilde{\omega}_0 = {\rm FW\_point}(D[Y==0])$
\State $\Tilde{\omega}_1 = {\rm FW\_point}(D[Y==1])$
\State $\Hat{\sigma} = \argmax_{\sigma > 0} l(\Tilde{\omega}_0,\Tilde{\omega}_1,\sigma| D,Y)$ with root solving.
\State {\bf Output: } $(\Tilde{\omega}_0,\Tilde{\omega}_1,\Hat{\sigma})$
\end{algorithmic}
\end{algorithm}



==> tropical_inner_product.tex <==
\section{Tropical Arithmetics and Tropical Inner Product}\label{Sec:tro:inner:prod}

In tropical geometry, addition and multiplication are different than
regular arithmetic. 
The arithmetic operations are performed
in the
max-plus tropical semiring $(\,\mathbb{R} \cup \{-\infty\},\oplus,\odot)\,$
as defined in \cite{pin1998tropical}. 
\begin{definition}[Tropical Arithmetic Operations]
  In the tropical semiring, the basic tropical
  arithmetic operations of addition and multiplication are defined as:
  $$a \oplus b := \max\{a, b\}, ~~~~ a \odot b := a + b, ~~~~\mbox{  where } a, b \in \mathbb{R}\cup\{-\infty\}.$$
  The element $-\infty$ ought to be included as it is the 
  identity element of tropical addition.
  Tropical subtraction is not well-defined and tropical division is classical subtraction.
\end{definition}

The following definitions are necessary for the definition of the tropical inner product
\begin{definition}[Tropical Scalar Multiplication and Vector Addition]
  For any scalars $a,b \in \mathbb{R}\cup \{-\infty\}$ and for any vectors 
  $v,w \in (\mathbb{R}\cup\{-\infty\})^e$, 
  where $e \in \mathbb{N}$, %is the dimension of the space,
 %  tropical scalar multiplication and tropical vector addition 
 % is defined as follows:
    \begin{align*}
        a \odot & v:= (a + v_1,  \ldots ,a + v_e), \\ 
        a \odot v  \oplus b \odot w &:= (\max\{a+v_1,b+w_1\}, \ldots, \max\{a+v_e,b+w_e\}).
    \end{align*}
\end{definition}
From the definitions above, it follows that the tropical inner product is
$\omega^T \odot x = \max \{ \omega + x \}$ 
for all vectors $\omega,x \in \trtor$.
In classical logistic regression a linear function in the form of a classical inner product 
$h_{\omega}(x) = \omega^T x, \, \omega \in \R^n $ is used.
The tropical symbolic equivalent is 
\begin{equation}
    \label{eq:h_omega_trop}
    h_{\omega}(x) = \omega^T \odot x = \max_{l \in [e]} \{ \omega_l + x_l \}.
\end{equation}
This expression is not well-defined, since the statistical parameter and covariate
vectors $\omega, u \in \mathbb{R}^e / \mathbb R {\rm 1} $ are only defined up to 
addition of a scalar multiple of the vector $(1,\dots,1)$.
To resolve this issue, we fix 
\begin{equation}
    \label{eq:fix_min}
    - \min_{l \in [e]} \{ \omega_l + x_l  \} = c, 
\end{equation}  
where $c \in \R$ is a constant for all observations. 
Combining equations \eqref{eq:fix_min}, \eqref{eq:h_omega_trop}, and the definition 
of tropical distance \eqref{eq:tropmetric}, 
\begin{equation*}
    h_{\omega}(x) = d_{\rm tr}(x,-\omega) - c. 
\end{equation*}
For simplicity, under the transformation $-\omega \to \omega$ the expression becomes
\begin{equation}
    \label{eq:h_omega}
    h_{\omega}(x) = d_{\rm tr}(x,\omega) - c. 
\end{equation}
% The interpretation of the statistical parameter $\omega$ is that it represents the 
% species tree of the class $Y=0$, 
% while the covariates $x$ represent the sampled 
% gene trees. If a sampled tree has a small tropical distance from the species tree of 
% the class $Y=0$, then $h_{\omega}$ is small. 
% In particular, the classifier for this model is 
% \begin{equation*}
%     C(x) = \mathbb{I}\left(
%         d_{\rm  tr}( x , \omega) > c
%     \right),
% \end{equation*}
% where to have a non-trivial classifier it 
% is required that $c>0$.

==> ult_thm.tex <==
\section{Space of ultrametrics} \label{sec:ult_thm}
\begin{theorem}[explained in \cite{AK,10.1093/bioinformatics/btaa564}] \label{thm}
Suppose we have a {\em classical} linear subspace $L_m \subset \RR^e$ defined by the linear
equations $x_{ij} - x_{ik} + x_{jk}=0$ for $1\leq i < j <k \leq m$. Let $\mbox{Trop}(L_m)\subseteq \RR^e/\RR {\bf 1}$ be the {\em tropicalization} of the linear space $L_m \subset \RR^e$, that is, 
classical operators are replaced by tropical ones (defined in Section \ref{Sec:tro:inner:prod} in the supplement)
in the equations defining the linear subspace $L_m$, so that all points $(v_{12},v_{13},\ldots, v_{m-1,m})$ in $\Trop(L_m)$ satisfy the condition that 
\[
\max_{i,j,k\in [m]}\{v_{ij},v_{ik},v_{jk}\}.
\]
is attained at least twice.
Then, the image of $\Tn$ inside of the tropical projective torus $\RR^e/\RR {\bf 1}$ is equal to $\Trop(L_m)$. 
\end{theorem}
